Leveraging Visemes for Better Visual Speech Representation and Lip Reading

Lip reading is a challenging task that has many potential applications in speech recognition, human-computer interaction, and security systems. However, existing lip reading systems often suffer from low accuracy due to the limitations of video features. In this paper, we propose a novel approach that leverages visemes, which are groups of phonetically similar lip shapes, to extract more discriminative and robust video features for lip reading. We evaluate our approach on various tasks, including word-level and sentence-level lip reading, and audiovisual speech recognition using the Arman-AV dataset, a largescale Persian corpus. Our experimental results show that our viseme based approach consistently outperforms the state-of-theart methods in all these tasks. The proposed method reduces the lip-reading word error rate (WER) by 9.1% relative to the best previous method.

==> end/appendices.tex <==
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.



==> end/bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:



% if you will not have a photo at all:


% insert where needed to balance the two columns on the last page with
% biographies
%\newpage



% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> end/ref.tex <==
% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}
	
	\bibitem{IEEEhowto:kopka}
	H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
	0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
	
\end{thebibliography}


==> first/abs.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}

% Due to its potential applications in fields such as speech recognition, human-computer interaction, and security systems, lip reading has garnered substantial attention in recent years as a challenging task. In this paper, we propose a novel viseme-based approach to improve the accuracy of lip reading systems by extracting better video features. The resulting model can be used in problems where we want to use visual features. We conducted several experiments to evaluate the effectiveness of our proposed approach, including word-level and sentence-level lip reading, as well as audio-visual speech recognition using the Arman-AV dataset. Throughout all these experiments, the produced model consistently achieves improved accuracy.

Lip reading is a challenging task that has many potential applications in speech recognition, human-computer interaction, and security systems. However, existing lip reading systems often suffer from low accuracy due to the limitations of video features. In this paper, we propose a novel approach that leverages visemes, which are groups of phonetically similar lip shapes, to extract more discriminative and robust video features for lip reading. We evaluate our approach on various tasks, including word-level and sentence-level lip reading, and audio-visual speech recognition using the Arman-AV dataset, a large-scale Persian corpus. Our experimental results show that our viseme based approach consistently outperforms the state-of-the-art methods in all these tasks. The proposed method reduces the lip-reading word error rate (WER) by 9.1\% relative to the best previous method.

\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010178.10010224</concept_id>
       <concept_desc>Computing methodologies~Computer vision</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

% \ccsdesc[500]{Computing methodologies~Computer vision}


%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{
    Visemes,
    Lip reading,
    Visual speech representation,
    Audio-visual speech recognition,
    Arman-AV dataset
}



% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
% \IEEEpeerreviewmaketitle

==> first/authors.tex <==
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{Ben Trovato}
% \authornote{Both authors contributed equally to this research.}
% \email{trovato@corporation.com}
% \orcid{1234-5678-9012}
% \author{G.K.M. Tobin}
% \authornotemark[1]
% \email{webmaster@marysville-ohio.com}
% \affiliation{%
%   \institution{Institute for Clarity in Documentation}
%   \streetaddress{P.O. Box 1212}
%   \city{Dublin}
%   \state{Ohio}
%   \country{USA}
%   \postcode{43017-6221}
% }

\author{Javad Peymanfard}
\affiliation{%
  \institution{Iran University of Science and Technology}
  \city{Tehran}
  \country{Iran}}
\email{javad\_peymanfard@comp.iust.ac.ir}

\author{Vahid Saeedi}
\affiliation{%
  \institution{Iran University of Science and Technology}
  \city{Tehran}
  \country{Iran}}
\email{vahid\_saeedi@alumni.iust.ac.ir}

\author{Mohammad Reza Mohammadi}
\affiliation{%
  \institution{Iran University of Science and Technology}
  \city{Tehran}
  \country{Iran}}
\email{mrmohammadi@iust.ac.ir}

\author{Hossein Zeinali}
\affiliation{%
  \institution{Amirkabir University of Technology}
  \city{Tehran}
  \country{Iran}}
\email{hzeinali@aut.ac.ir}

\author{Nasser Mozayani}
\affiliation{%
  \institution{Iran University of Science and Technology}
  \city{Tehran}
  \country{Iran}}
\email{mozayani@iust.ac.ir}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\shortauthors}{Peymanfard et al.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \author{Valerie B\'eranger}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }

% \author{Aparna Patel}
% \affiliation{%
%  \institution{Rajiv Gandhi University}
%  \streetaddress{Rono-Hills}
%  \city{Doimukh}
%  \state{Arunachal Pradesh}
%  \country{India}}

% \author{Huifen Chan}
% \affiliation{%
%   \institution{Tsinghua University}
%   \streetaddress{30 Shuangqing Rd}
%   \city{Haidian Qu}
%   \state{Beijing Shi}
%   \country{China}}

% \author{Charles Palmer}
% \affiliation{%
%   \institution{Palmer Research Laboratories}
%   \streetaddress{8600 Datapoint Drive}
%   \city{San Antonio}
%   \state{Texas}
%   \country{USA}
%   \postcode{78229}}
% \email{cpalmer@prl.com}

% \author{John Smith}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}}
% \email{jsmith@affiliation.org}

% \author{Julius P. Kumquat}
% \affiliation{%
%   \institution{The Kumquat Consortium}
%   \city{New York}
%   \country{USA}}
% \email{jpkumquat@consortium.net}















% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%

%\author{Michael~Shell,~\IEEEmembership{Member,~IEEE,}
%	John~Doe,~\IEEEmembership{Fellow,~OSA,}
%	and~Jane~Doe,~\IEEEmembership{Life~Fellow,~IEEE}% <-this % stops a space
%	\thanks{M. Shell was with the Department
%		of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta,
%		GA, 30332 USA e-mail: (see http://www.michaelshell.org/contact.html).}% <-this % stops a space
%	\thanks{J. Doe and J. Doe are with Anonymous University.}% <-this % stops a space
%	\thanks{Manuscript received April 19, 2005; revised August 26, 2015.}}

% \author{\IEEEauthorblockN{1\textsuperscript{st} Javad~Peymanfard}
% \IEEEauthorblockA{\small{School of Computer Engineering} \\
% \small{Iran University of Science and Technology}\\
% Tehran, Iran \\
% javad\_peymanfard@comp.iust.ac.ir}
% \and
% \IEEEauthorblockN{2\textsuperscript{nd} Vahid~Saeedi}
% \IEEEauthorblockA{\small{School of Computer Engineering} \\
% \small{Iran University of Science and Technology}\\
% Tehran, Iran \\
% vahid\_saeedi@alumni.iust.ac.ir}
% \and
% \IEEEauthorblockN{3\textsuperscript{rd} Mohammad Reza Mohammadi}
% \IEEEauthorblockA{\small{School of Computer Engineering} \\
% \small{Iran University of Science and Technology}\\
% Tehran, Iran \\
% mrmohammadi@iust.ac.ir}
% \and
% \IEEEauthorblockN{4\textsuperscript{th} Hossein Zeinali}
% \IEEEauthorblockA{\small{Department of Computer Engineering} \\
% \small{Amirkabir University of Technology}\\
% Tehran, Iran \\
% hzeinali@aut.ac.ir}
% \and
% \IEEEauthorblockN{5\textsuperscript{th} Nasser Mozayani}
% \IEEEauthorblockA{\small{School of Computer Engineering} \\
% \small{Iran University of Science and Technology}\\
% Tehran, Iran \\
% mozayani@iust.ac.ir}
% }

% \author{
% Jefferson Santiago$^{1}$, Jes\'us Ar\'evalo$^{2}$, Luinel Andrade$^{3}$\\
% \small{$^{1-3}$Escuela de Computaci\'on, Facultad de Ciencias}\\
% \small{Universidad Central de Venezuela, 1024, Caracas, Venezuela.}\\
% \small{\texttt{\{$^{1}$jefri.26.4, $^{2}$jaas1710@, $^{3}$luinel1393\}@gmail.com}} %$^{3}$lex@fechorias.com}}
% }

% \author{\IEEEauthorblockN{Jefferson Santiago}
% \IEEEauthorblockA{Escuela de Computaci\'on\\Facultad de Ciencias\\
% Universidad Central de Venezuela\\
% Caracas, Venezuela\\
% Email: jefri.26.4@gmail.com}
% \and
% \IEEEauthorblockN{Jes\'us Ar\'evalo}
% \IEEEauthorblockA{Escuela de Computaci\'on\\Facultad de Ciencias\\
% Universidad Central de Venezuela\\
% Caracas, Venezuela\\
% Email: jaas1710@gmail.com}
% \and
% \IEEEauthorblockN{Luinel Andrade}
% \IEEEauthorblockA{Escuela de Computaci\'on\\Facultad de Ciencias\\
% Universidad Central de Venezuela\\
% Caracas, Venezuela\\
% Email: luinel1393@gmail.com}}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.


==> first/headers.tex <==
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
% 
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.




% If you want to put a publisher's ID mark on the page you can do it like
% this:
%\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.



% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}


==> intro/sub.tex <==
\subsection{Subsection Heading Here}
Subsection text here.


==> intro/subsub.tex <==
\subsubsection{Subsubsection Heading Here}
Subsubsection text here.

